JustFit: Just-in-Time State Management for Local LLM Serving

Local agents need memory for model execution and working history. We present JustFit, an MLX runtime that coordinates their overlapping allocations: KVExec executes and checkpoints four-bit KV with bounded workspace, PhaseSwap loads phase-dependent components, and StateTrans preserves history across execution modes. With Qwen3.8-27B MXFP4 on a 24 GiB M4 Pro MacBook, JustFit reaches 327,680 retained positions across two requests, 10.67 times the evaluated baseline's 30,720-position single-request record. One request completes the full 262,144-position native window at median 5.986 tokens/s. Each shape completes 16,384 outputs per request in three fresh processes: B1 uses one cold build and two prefix extensions; B2 uses three ordered prefix extensions (Section 4). Image encoding can proceed while preserving a live 196,608-input text request. A controlled, repetitive 32K+6K workload reaches median 18.284 tokens/s at 15,626 MiB; a separate AIME 2026 evaluation scores 29/30. Coordinating execution and state lifetimes makes longer histories feasible on personal hardware.

==> data/generated/b2_rows.tex <==
1 & 153,600 / 131,071 & 10,240 / 1 & 9.732 & 20,953 & 47 \\
2 & 163,839 / 131,071 & 1 / 1 & 9.738 & 20,456 & 544 \\
3 & 163,839 / 131,071 & 1 / 1 & 9.735 & 20,432 & 568 \\


==> data/generated/capacity_summary_rows.tex <==
B1: 256K & 3/3 & 5.986 & 20,357--20,450 \\
B2: 288K & 1/1 & 10.341 & 20,858 \\
B2: 320K & 3/3 & 9.735 & 20,432--20,953 \\


==> data/generated/dispersion_rows.tex <==
1 & 18,221--18,227 & 109.912--110.840 & 5.973--5.980 \\
2 & 18,099--18,220 & 115.858--115.862 & 6.539--6.542 \\
3 & 17,795--17,806 & 115.878--115.889 & 13.288--13.294 \\
4 & 17,040--17,051 & 110.559--110.578 & 11.441--11.446 \\
5 & 16,545--16,559 & 110.549--110.560 & 11.445--11.445 \\
6 & 16,365--16,403 & 108.850--108.877 & 11.539--11.545 \\
7 & 16,364--16,405 & 115.006--115.012 & 11.534--11.539 \\
8 & 15,630--15,632 & 114.567--114.747 & 18.269--18.277 \\
9 & 15,632--15,632 & 113.738--114.408 & 18.289--18.298 \\
10 & 15,626--15,640 & 114.338--114.375 & 18.271--18.393 \\


==> data/generated/evolution_rows.tex <==
0 & mlx-vlm baseline & 30K (B1) & $21{,}000\,\times$ & --- & --- \\
1 & TQ4 + MTP & 38K & 18,225 & 110.82 & 5.975 \\
2 & Fused dequant & 80K & 18,220 & 115.86 & 6.541 \\
3 & Segmented KV & 128K & 17,806 & 115.89 & 13.291 \\
4 & Paged KV + attention & 128K (carried) & 17,044 & 110.57 & 11.446 \\
5 & Page-native MTP + lifecycle & 159K & 16,547 & 110.55 & 11.445 \\
6 & Eager release + scheduling & 208K & 16,374 & 108.88 & 11.541 \\
7 & Direct-inverse prefill & 224K (B2) & 16,365 & 115.01 & 11.539 \\
8 & Optimized verifier & 208K (B1) & 15,631 & 114.71 & 18.275 \\
9 & Head-grouped prefill & --- & 15,632 & 114.36 & 18.292 \\
10 & Borrowed APC + single-pass writer & 256K B1; 320K B2 & 15,626 & 114.37 & 18.284 \\


==> data/generated/head_group_rows.tex <==
32K & 44.752 & 42.180 & 526.1 & 268.6 \\
96K & 132.024 & 136.474 & 1,566.4 & 796.9 \\
192K & 271.220 & 280.897 & 3,123.8 & 1,589.3 \\


==> data/generated/m3_comparison_rows.tex <==
B1 32K+6K ($n=3$) & 87.109 & 114.373 & 12.603 & 18.284 & 15{,}650 & 15{,}626 \\
B1 cold 240K+16K & 44.403 & 60.546 & 4.944 & 5.936 & 20{,}905 & 20{,}357 \\
B2 cold $2\times$(128K+16K) & 57.262 & 81.399 & 7.101 & 10.341 & 20{,}749 & 20{,}858 \\
B4 staggered, four lanes & 62.888 & 85.452 & 16.800 & 22.570 & 19{,}285 & 18{,}915 \\


==> data/generated/native_rows.tex <==
1 & Cold & 0 & 245,760 & 60.546 & 5.936 & 20,357 & 643 \\
2 & Checkpoint & 161,792 & 83,968 & 44.331 & 5.987 & 20,449 & 551 \\
3 & Checkpoint & 161,792 & 83,968 & 44.315 & 5.986 & 20,450 & 550 \\


==> data/generated/vision_all_rows.tex <==
98,304 & 98,303 & 1 & 143,360 & 20,700 & 20,346 & 354 & 16.419 \\
131,072 & 131,071 & 1 & 143,360 & 20,700 & 20,335 & 365 & 18.094 \\
163,840 & 163,839 & 1 & 204,800 & 21,000 & 20,635 & 365 & 19.873 \\
196,608 & 161,792 & 34,816 & 204,800 & 21,000 & 20,852 & 148 & 21.636 \\
200,704 & 194,560 & 6,144 & 204,800 & 21,000 & 20,980 & 20 & 12.994 \\


==> data/generated/vision_main_rows.tex <==
98,304 & 16.419 & 20,346 & 20,700 \\
131,072 & 18.094 & 20,335 & 20,700 \\
163,840 & 19.873 & 20,635 & 21,000 \\
196,608 & 21.636 & 20,852 & 21,000 \\


==> data/generated/vision_timing_rows.tex <==
98,304 & 2.385 & 1.735 \\
131,072 & 2.313 & 1.109 \\
163,840 & 2.685 & 1.130 \\
196,608 & 723.711 & 1.177 \\
200,704 & 140.741 & 1.187 \\


==> data/generated/writer_rows.tex <==
16K & 0.0872 & 0.0479 & 545,270,638 & 272,635,224 \\
32K & 0.1550 & 0.0869 & 1,090,530,364 & 545,265,080 \\
224K & 2.9759 & 1.5073 & 7,633,644,836 & 3,816,822,312 \\

